GRASP: Guiding model with RelAtional Semantics using Prompt for Dialogue Relation Extraction

The dialogue-based relation extraction (DialogRE) task aims to predict the relations between argument pairs that appear in dialogue. Most previous studies utilize fine-tuning pre-trained language models (PLMs) only with extensive features to supplement the low information density of the dialogue by multiple speakers. To effectively exploit inherent knowledge of PLMs without extra layers and consider scattered semantic cues on the relation between the arguments, we propose a Guiding model with RelAtional Semantics using Prompt (GRASP). We adopt a prompt-based fine-tuning approach and capture relational semantic clues of a given dialogue with 1) an argument-aware prompt marker strategy and 2) the relational clue detection task. In the experiments, GRASP achieves state-of-the-art performance in terms of both F1 and F1c scores on a DialogRE dataset even though our method only leverages PLMs without adding any extra layers.

==> sections/0_introduction.tex <==
\section{Introduction}
\label{intro}
\input{figures/prompt_example}

% - RE설명 & Cross Sentence RE 설명
% - Dialogue RE의 특수성
% 1) higher person pronoun frequency
% 2) lower information density

% Relation extraction task (RE) predicts the correct semantic relations between arguments from a text. As a large number of relational facts appear in multiple sentences, such as in a single document or dialogue, the importance of cross-sentence RE increases as well~\cite{yao2021codred}. With the significance of cross-sentence RE, dialog based relation extraction (DialogRE) entails additional difficulties due to the nature of a dialogue. The task of DialogRE aims to identify the relation between arguments by depending on the intrinsic relational cue rather than exploiting external knowledge~\cite{yu-etal-2020-dialogue}.
The relation extraction (RE) task aims to extract semantic relations from unstructured text such as a sentence, a document, or even a dialogue. RE plays a critical role in information extraction and knowledge base construction due to its capability to extract structured relational information \citep{ji2010overview,swampillai2010inter}. However, since a large number of relational facts appear across multiple sentences with more than one speaker in dialogue, utilizing sentence-level RE in a conversational setting is limited \citep{yao2021codred}. To encourage building a model that captures underlying semantics spread in the dialogue, dialog-based relation extraction (DialogRE) dataset emerges which includes argument pairs and their corresponding relation as in Table \ref{tab:dialogRE} \citep{yu-etal-2020-dialogue}. 
\input{tables/intro_dialogre}
Previous studies that have achieved state-of-the-art (SoTA) performance in DialogRE benchmarks exploit fine-tuning to the pre-trained language models (PLMs) \citep{lee-choi-2021-graph,ijcai2021-535} such as BERT \citep{devlin-etal-2019-bert} and RoBERTa \citep{liu2019roberta}. As fine-tuning requires adding extra layers on top of the PLMs and different training objectives from those used in the pre-training phase, PLMs are reluctant to exploit their learned knowledge in the downstream task resulting in less generalized capability \citep{chen2021knowprompt}. 
% 모델의 사전 학습 단계에서 범용적으로 학습한 지식을 다운스트림 테스크에서 제대로 활용하지 못한다, making it hard to generalize well \cite{}.
% their performance enormously relies on labor-intensive annotated data, making it hard to generalize well.
% training the models under task-specific objectives different from those used in the pre-training, 
% their performance enormously relies on labor-intensive annotated data, making it hard to generalize well.
% 그들의 성능은 objectives의 gap으로 인한 사전 학습 단계에서 학습한 지식을 제대로 활용하지 못한다.
% 사전 학습 단계와 미세 조정 단계의 차이는 사전 학습 단계에서 학습한 지식을 제대로 활용하지 못하기 때문에, 많은 양의 데이터에 의존한다.
% 모델의 사전 학습 단계에서 범용적으로 학습한 지식을 다운스트림 테스크에서 제대로 활용하지 못한다, making it hard to generalize well \cite{}.


For effective utilization of knowledge from PLMs, a series of studies using prompt-based fine-tuning employ the PLM directly as a predictor by completing a cloze task to bridge the gap between pre-training and fine-tuning \citep{gao2020making,han2021ptr,chen2021knowprompt}.
% Prompt-tuning 예제
As shown in Figure \ref{fig:finetune_prompt}, prompt-based fine-tuning treats the downstream task as a masked language modeling (MLM) problem by directly generating the textual response to a given template. In other words, prompt-based fine-tuning fuses the original input with the template to predict \texttt{[MASK]} and then maps the predicted label words to the corresponding task-specific class sets. 
% Moreover, these studies overwhelm the performance of fine-tuning approaches in both full-shot and few-shot setting.

% Conversational setting에서 모델의 잠재력을 끌어올리기 위해서 반드시 고려해야 하는 몇 가지 요소가 있다.
% Text classification에 대한 Prompt leanring의 성공에도 불구하고, 모델이 Conversational text를 잘 이해하고 유의미한 추론을 하기 위한 어려움이 여전히 남아 있다.
% 이들은 DRE에서 few-shot 성능은 뛰어났으니, full-shot 성능은 fine-tuning based 를 넘지 못한다 이유는..
Nevertheless, the previous studies using prompt-based fine-tuning are still not enough in performance than the fine-tuning based approach. We assume that this phenomenon is derived from the properties of conversation as follows: higher person pronoun frequency~\citep{wang2011pilot} and lower information density~\citep{biber1991variation} by multiple speakers\footnote{In DialogRE dataset, 65.9\% of relational triples involve arguments that never appear in the same utterance, demonstrating that multi-turn reasoning plays an important role.}. Therefore, a prompt-based fine-tuning approach that takes sparse semantics lying in the dialogue into account is required to improve the model's understanding capability of the relation between the arguments in the dialogue. 




% with consideration on the two challenging properties of dialogue is required further to improve the model's capability on the dialogue. Without consideration on the two properties, it is complicated to capture precise relations between the arguments from the dialogue.
% In DialogRE, 65.9\% of relational triples involve arguments that never appear in the same utterance, demonstrating that multi-turn reasoning plays an important role. For example, to predict that ``Alice" is a child of ``Leslie" in Table \ref{tab:dialogRE}, it is required to memorize a trigger ``kids" in the first turn until the last turn where ``Leslie" appears for the first time.

% we have to memorize a trigger ``kids" in the first turn until the last turn where ``Leslie" appears for the first time.
% Conversational texts have features including low information density, which makes the model hard to figure out which part of the dialogue is a clue for predicting an answer \cite{wang2011pilot}.

% Despite above rich and powerful features, it seems that the explicit information is not enough to capture the correct relation in performance level, implying that injecting fine-grained dialogue representation to the PLM meets an upper limit. Besides, in the process of fine-tuning PLM, the limitation of high computational cost with less effective performance gain still exists. At the same time, recent series of studies on prompt-tuning \cite{ding2021prompt,gu2021ppt,shen2021trigger,wu2021curriculum,zhang2017position,zhang2019long} find the way of deflecting the dead end by leveraging model's learned knowledge in straight manner. Because DialogRE can be solved with implicit semantics from the given dialogue~\cite{yu-etal-2020-dialogue}, nothing is needed except the relational clue with contextual comprehension of PLMs. Therefore, we adopt prompt learning to guide PLM for capturing intrinsic relation with its obtained knowledge during pre-training.
% 여러 Feature를 이용한 논문들 소개 
% In conversational setting, it has two major challenges of 1) higher person pronoun frequency~\cite{wang2011pilot} and 2) lower information density~\cite{biber1991variation} by multiple speakers. Due to these two obstacles, it is complicated to capture precise relations of arguments from the dialogue. The strong baseline introduced along with the DialogRE dataset considers \textit{speaker information} by token-replacement encoding strategy that takes account of only speakers rather than other arguments. Owing to its limited coverage, the abundant amount of useful information still remains intact. To extract such information from the dialogue, there are the approaches that focus on \textit{trigger}, which indicates the existence of the relation between two arguments~\cite{xue2021gdpnet,zhang2021improving}. In addition, Lee and Choi~\shortcite{lee-choi-2021-graph} concentrate on \textit{turn information} by a heterogeneous dialogue graph including four different types of nodes and three dissimilar types of edges and leverages graph convolutional network (GCN) \cite{kipf2016semi} with pre-trained language model (PLM) to predict the relation.

% Moreover, another considers \textit{speaker information} utilizing masking strategies refining multi-grained word representation from the PLM and mutual attention aggregating entity representations~\cite{ijcai2021-535}.


% % 다른 피쳐를 쓴 논문 제목 두개만 알려주소 GDPNet, Semantic Representation for Dialogue Modeling"
% Trigger 인식 모델: From What to Why: Improving Relation Extraction with Rationale Graph
% The reason that utilizing multiple rich information has limitation on performance is attribute to task properties. 
% complexity 도 (부차적으로) 높은 것도 단점.


% BERTs 의 출현 이유.
% arguments 와 relavant 한 turns 를 모델에게 help to locate 하기 위해,(speaker 에 기반해서)
% BERTs 는 given dialogue 의 speaker information 을 고려하는 인코딩 전략을 제안한다. 이는 관계 예측을 위해 대화와 함께 주어진 arguments가 발화자라면 토큰 치환을 통해서 speaker의 intensity? semantics?를 증대시키고, 오버피팅을 방지하기 위해서 제안된 메소드이다. 그런데, 이는 발화자만(speaker)만을 고려하기 때문에 non-speaker인 arguments에 대한 고려가 부족하다.

% - 내재적인 관계 정보를 포착하는 것이 가장 중요한 DRE 태스크를 위해, 우리는 PLM 의 지식의 활용을 최대화할 수 있는 Promt-tuning 방법론을 follow 한다. 또한, prompt-tuning 을 통해, 추가적 레이어 없이 light-weight 학습 방법론을 유지함으로써, 앞선 모델들의 heavy complexity 문제도 해결하고자 한다.

% 이러한 PLM의 지식을 최대화하는 prompt-tuning 방법론은 앞서 언급한 DRE 태스크의 어려움을 해결하는데 leaverage할 수 있다.

% RE는 외부 지식으로 도움받을 수 있는데, DRE는 문맥에 대한 이해 능력으로 추론함. PT 모델에게 방대한 코퍼스로 문맥 이해 능력을 부여 -> FT PT gap 때문에 PT에서의 문맥 이해 능력 손실 -> DRE 테스크 특성이 FT로는 한계가 있다 :

% model's capability of leveraging its learned. 
% To lift the burden on PLM's shoulder with the full advantage of PLM's intrinsic knowledge directly, we adopt prompt learning by suggesting an additional task for dialogueRE.  
% by bridging the gap of objective forms in pre-training and fine-tuning~\cite{chen2021knowprompt}. 

% Additionally, our approach using prompt-learning also gets advantages of light-weight training simultaneously.
We propose the method of \textbf{G}uiding model with \textbf{R}el\textbf{A}tional \textbf{S}emantics using \textbf{P}rompt learning for DialogRE ($\mathbf{GRASP}$). In order to get advantages of prompt-based fine-tuning approach as much as possible for DialogRE task, we suggest argument-aware prompt marking (APM) strategy and relational clue detection (RCD) objective. 
APM strategy is to guide the model to the significant arguments scattered in the dialogue by carefully considering both speaker and non-speaker arguments. 
% In other words, we expand the previous baseline called BERT${_s}$ to navigate broadened coverage of arguments in the dialogue.
Along with our APM strategy, we suggest the RCD task with a training objective that leads the model to pay attention to the significant relational clues. Specifically, the model is trained to discriminate whether each token in a dialogue belongs to a subject, object, or trigger. As a result, we let the PLM train on RCD and MLM altogether. 
From our experiments, our method achieves SoTA performances in DialogRE task for both full-shot and few-shot settings at a substantial level. By employing only PLMs without adding an extra layer as a predictor,  $\mathbf{GRASP}$ demonstrates the higher performances than other baselines, implying attending to significant semantic clues guides the PLMs to predict correct relation with its inherent knowledge. Moreover, we provide ablation studies and analyses on whether our method drives the model on the relational cues more than before.


Our contributions are as follows:
\begin{itemize}
\item {We adopt a prompt-based fine-tuning approach to utilize PLM's inherent knowledge directly for dialogue where the information density is relatively low.}

\item {We introduce an argument-aware prompt marking (APM) strategy and relational clue detection (RCD) task to guide PLMs on the significant relational clues to predict relation.}

\item {We demonstrate that our proposed method achieves SoTA in the DialogRE task and provide detailed analyses of the effectiveness of our approach.}

\end{itemize} 


% speaker 및 다른 피쳐를 쓰는데도 왜 성능 안올라 -> prompt-tuning이 DRE에 더 맞다고 생각하는 이유가: RE는 외부 지식으로 도움받을 수 있는데, DRE는 문맥에 대한 이해 능력으로 추론함. PT 모델에게 방대한 코퍼스로 문맥 이해 능력을 부여 -> FT PT gap 때문에 PT에서의 문맥 이해 능력 손실 -> DRE 테스크 특성이 FT로는 한계가 있다 : intrinsic semantic information for relation 
% + 추가적인 레이어 없이 Light-weight 을 유지함으로써, pLM의 지식을 최대화 하는 것으로 가성비 좋은 성능을 내겠다.

% adopting the pre-trained
% LM directly as a predictor by completing a cloze task to bridge
% the gap between pre-training and fine-tuning. Prompt-tuning fuses
% the original input with the prompt template to predict [MASK] and
% then maps the predicted label words to the corresponding class sets,
% which has induced better performances for PLMs on few-shot tasks.
% Prompt-tuning fuses
% the original input with the prompt template to predict [MASK] and
% then maps the predicted label words to the corresponding class sets,
% which has induced better performances for PLMs on few-shot tasks.


% - 기존의 approach 설명 앤드 까기 
% 1) TUCORE-GCN - lm + rich graph representation (subject object)
% 2) COIN - language model + masking strategy (speaker focused)


% dialogue re 태스크에서의 Relational clue (뒤에서 $R_{clue}$ 로 나올거) 의 중요성에 대한 역설이 강조되어야함.
% $\to$ 어떤 대화의 sparsity 를 이야기하면서, ``So, what should we pay attention to?" 에 대한 질문에 ``바로바로 relational clue"야. 라고 대답하는 것이 우리의 중헌 motivation 임.


==> sections/2_method.tex <==
\input{figures/overview_figure}

\section{Methodology}
An overview of $\mathbf{GRASP}$ is illustrated in Figure \ref{fig:model_overview}. We first construct input with a prompt template and APM strategy. Then PLM receives the input for prompt-based fine-tuning and outputs probability distributions over the model's vocabulary from contextualized representations of PLM. While the model trains with the RCD task by predicting the relational clue type of each token, MLM takes \texttt{[MASK]} representation to predict a final relation. In other words, we train our model in a multi-tasking manner to encourage the model's mutual communication between relational clues and the final relation for the argument pair. 

% In this section, we provide a detailed explanation of our proposed method and introduce our overall framework as in Figure \ref{fig:model_overview}. After constructing input with a prompt template and argument-aware prompt marking (APM) strategy, PLM receives the input for prompt-based learning. Then the softmax function~\cite{bridle1989training} outputs probability distributions over the model's vocabulary from contextualized representations of PLM. While RCD trains the model by taking each token to detect a type of relational clues, MLM takes \texttt{[MASK]} the representation to predict a final relation. In other words, we train our model in a multi-tasking manner to encourage the model's mutual communication between relational clues and the final relation for the argument pair. 

\subsection{Problem Formulation}
\label{subsec:problem_formulation}
% The DialogRE dataset consists of \{$\mathcal{X}$, $\mathcal{Y}$\}, where $\mathcal{X}$ is the set of examples and $\mathcal{Y}$ is corresponding labels. 
Each example $\mathcal{X}$ includes a dialogue $D$, subject $a_1$, object $a_2$. Note that $D$ denotes $\{s_1:u_1, s_2:u_2,\dots,s_N:u_N\}$, where $u_n$ is $n$-th utterance and $s_n$ is the corresponding speaker. Given $\mathcal{X}=\{D,a_1,a_2\}$, the goal of DialogRE is to predict the relation $y$ between the arguments $a_1$ and $a_2$ by leveraging $D$. To describe the DialogRE task in terms of prompt-based learning, we define template function $\mathcal{T}(\cdot)$ as below. It is utilized to map each example to construct an input $\mathcal{X}_{prompt}=\mathcal{T}(\mathcal{X})$. 
A \texttt{[MASK]} is inserted into $\mathcal{X}_{prompt}$ to predict the label words of the relation $y$. The formulation of $\mathcal{T}(\mathcal{X})$ is as follows:
\begin{equation}\label{eq:prompt_design}
\scalebox{0.88}{$
\begin{aligned}
     \mathcal{T}(\mathcal{X}) = 
    \text{``}&\texttt{[CLS]} D \texttt{[SEP]} \texttt{[subj]} a_1 \texttt{[subj]} \\
    &\texttt{[MASK]} \texttt{[obj]} a_2 \texttt{[obj]} \texttt{[SEP]}\text{"}.
\end{aligned}
$}
\end{equation}
% In addition, to model the comprehension of PLM on the relational clues, we denote $R_{clue}^{\mathcal{X}}$ for each example $\mathcal{X}$ as $\{a{_1},~a{_2},~trigger\}$ regarded as the relational clues to predict the relation between the arguments.
Based on the structure of $\mathcal{T}(\cdot)$, we construct our template function $\mathcal{T}'(\cdot)$ 
by applying two steps; transformation of $D$ to $D'$ with an argument-aware prompt marker in \ref{subsection:encoding}, and a prompt initialization for \texttt{[subj]},\texttt{[obj]} in \ref{subsection:prompt}.
Afterwards, we introduce RCD task in \ref{subsection:rcd}, and train the model by utilizing $\mathcal{T}'(\cdot)$ with a multi-task training strategy on MLM in \ref{subsec:model_training}.

% Consequently, the $\mathcal{T}(\cdot)$ is to be redefined in the form of T'(\cdot). Each of our strategies for the components of $\mathcal{T'}(\cdot)$ is explained individually in each following subsection.

% 1. 데이터 관점 : encoding strategy
% 2. Model 관점 : RCD task

\subsection{Argument-aware Prompt Marker}
\label{subsection:encoding}
% 들어갈 내용
% 이전 입력 인코딩 단계의 argument 고려는 speaker token에 대한 replacement 방법론인 BERTs이다. 하지만 추가적인 feature 없이 모델의 argument awareness를 향상시키기 위해서 우리는 non-speaker argument도 고려해야 함
We propose an argument-aware prompt marking (APM) strategy that considers both speaker and non-speaker arguments. 
Previous studies that encode a dialogue by focusing on the speaker information~\cite{lee-choi-2021-graph,yu-etal-2020-dialogue,chen2021knowprompt} lack consideration of the non-speaker arguments. However, in the DialogRE dataset, approximately 77.4\% of relation triples include at least one non-speaker argument, implying that consideration of the non-speaker arguments is also required to enhance the model's argument-awareness.


Inspired by previous work of \citet{soares2019matching} and \citet{han2021ptr}, we insert argument-aware prompt marker token \texttt{[p]} as an entity marker; the former addresses the importance of entity markers regarding recognition of the entity position, and the latter improves the model performance by using specific additional punctuation in the model's original vocabulary as the entity marker.  
% Prompt marker 가 기존 entity marker 보다 더 좋은 이유 (기대 효과)
From our argument-aware prompt markers, we let our model obtain informative signs to discriminate which token is the indicative component for the relation prediction.
We initialize the feature of \texttt{[p]} as the embedding of space token in the model's vocabulary. Based on our empirical experiments, it turns out that the space token is well applicable to perceive the start position of the arguments. Accordingly, our prompt marker enhances the model to discriminate which part of dialogue plays a critical role in predicting a relation.
% is a start token among the subwords divided by a tokenization algorithm such as byte pair encoding (BPE)~\citep{sennrich2015neural}.

With the suggested argument-aware prompt marker, we strengthen the token replacement method of BERT${_s}$~\citep{yu-etal-2020-dialogue}. 
% APM is the advanced version of the token replacement method of BERT${_s}$ \citep{yu-etal-2020-dialogue}. 
% % BERT${_s}$ 의 방식은 다음과 같다.
Given an example $\mathcal{X}$, BERT${_s}$ constructs $\tilde{\mathcal{X}} = \{\tilde{D},\tilde{a_1},\tilde{a_2}\}$, where $\tilde{D} = \{ \tilde{s}_1:u_1, \tilde{s}_2:u_2, \dots, \tilde{s}_N:u_N \}$ and $\tilde{s_n}$ is:
\begin{equation}
{
    \tilde{s_n} = \begin{cases} 
    \texttt{[S$_1$]} & $if$\ s_n=a_1 \\
    \texttt{[S$_2$]} & $if$\ s_n=a_2 \\
    s_n & $otherwise$
    \end{cases}
} 
\end{equation} \label{equation:berts}
\texttt{[S$_1$]} and \texttt{[S$_2$]} are special tokens for speakers. In addition, $\tilde{a}_m$ ($m\in\{1,2\}$) is defined as \texttt{[S$_m$]} if $\exists~n~(s_n=a_m)$, and $a_m$ otherwise. 

Even though BERT${_s}$ prevents the model from overfitting and shows higher generalization capacity~\citep{yu-etal-2020-dialogue}, BERT${_s}$ lacks the consideration of the non-speaker arguments. To explore these unregarded arguments, the APM strategy expands BERT$_s$, with the consideration on both types of arguments for the DialogRE task.
We define a function \texttt{APM($\cdot$)} that encodes a utterance by inserting \texttt{[p]} in front of each argument token. Given a dialogue $\tilde{D}$ constructed by BERT$_s$, 
we construct $D' = \{\tilde{s}_1:u'_1, \tilde{s}_2:u'_2, \dots, \tilde{s}_N:u'_N\}$ by applying \texttt{APM}$(u_n)$ for each utterance in $\tilde{D}$. 
As a result, APM strategy constructs $\mathcal{X}' = \{D',\tilde{a}_1, \tilde{a}_2\}$ based on $\mathcal{\tilde{X}}$.
\begin{equation}
{
    \scalebox{0.85}{$u'_n = \begin{cases}
    \texttt{APM}(u_n) & $if$~\exists~m~(\tilde{a}_m \in u_n)~(m \in \{1,2\}) \\
    u_n & $otherwise$
    \end{cases}$}
}
\end{equation}
For instance, $\texttt{APM}(\cdot)$ encodes the text ``I am Tom Gordon" to \texttt{[I, am, [p], Tom, Gordon]}, inserting \texttt{[p]} in front of ``Tom Gordon". 

\subsection{Prompt Construction}
\label{subsection:prompt}
% 들어갈 내용
% 0. input design 의 각 구성 요소에 대한 설명.
% 1. Entity Type prior knowledge
% 2. Relation prior knowledge
% 3. base template (Figure with RCD)

% Our input sequence consists of dialogue, argument pair, prompt tokens for each argument type, and \texttt{[MASK]} token for relation prediction.


% RCD -> MLM(Final)
% The components required for RCD task are 

% The input design for MLM is ~. In this stage, we follow the prompt design of 노롬프트 model as the base 

% % 0번
% We follow the prompt design of KnowPrompt model as the base prompt structure.
% % 우리 빅풋 구조가 어떻게 생겼는가?
% As shown in the figure \ref{fig:model_overview}, input sequence consists of dialogue, argument pair, prompt tokens for each entity type, and mask token for prediction. 

% Followed by Yu et al.~\shortcite{yu-etal-2020-dialogue} and 

Inspired by \citet{chen2021knowprompt}'s work, we utilize prior distribution of argument types for deliberate initialization. The prompt tokens \texttt{[subj]} and \texttt{[obj]} are used to inject argument type information. We define the argument type set $\mathcal{AT}=\{$`PER', `ORG', `GPE', `VALUE', `STRING'$\}$ using the types pre-defined in the dataset as depicted in Table \ref{tab:dialogRE}. We calculate the distribution of argument types $\phi^{\texttt{[subj]}}$ and $\phi^{\texttt{[obj]}}$ over $\mathcal{AT}$ by frequency statistics, respectively.
We aggregate each argument type $at\in\mathcal{AT}$ with corresponding prior distribution to initialize the prompt tokens \texttt{[subj]} and \texttt{[obj]}. The specific initialization equations are as follows:
\begin{equation}
    \scalebox{0.9}{$
    \begin{aligned}
        \check{e}(\text{\texttt{[subj]}}) & = \sum_{at~\in \mathcal{AT}}{ \phi^{\texttt{[subj]}}_{at} \cdot e(at) } \\
        \check{e}(\texttt{[obj]}) & = \sum_{at~\in \mathcal{AT}}{ \phi^{\texttt{[obj]}}_{at} \cdot e(at) },
    \end{aligned}
    $}
\end{equation}
where $e(\cdot)$ is the embeddi from PLM of an input token, and $\check{e}(\cdot)$ is an initialized embedding of prompt token.
% , and $\phi^{\texttt{[subj]}}$ and $\phi^{\texttt{[obj]}}$ are the distribution over the candidate set $\mathcal{A}$.
% [figure 1= 데이터 내의 예시 문장들] + prior distribution의 예시를 한번에 해결
Suppose subject has prior distribution $\phi^{\texttt{[subj]}}=\{$`PER'$:0.5, $`ORG'$:$0.5, `GPE':$0.0, $`VALUE':$0.0, $`STRING':$0.0$\}.  The initial embedding of $\texttt{[subj]}$ token can be calculated as weighted average, i.e., $\check{e}(\texttt{[subj]}) = 0.5 \cdot e($`PER'$) + 0.5 \cdot  e$(`ORG'$)$.
% initialization for relation representation
In addition, to enhance the model's comprehension of each relation, we utilize its metadata for initialization of relation representation as well. 
For instance, to inject relational semantics of ``per:date\_of\_birth" into the model, we add a special token \texttt{[per:data\_of\_birth]} as corresponding relation \textit{label words} to the model's vocabulary and initialize this token by aggregating the embeddings of the tokens in metadata, i.e., \{`person', `date', `of', `birth'\}. 

Consequently, we can formalize $\mathcal{T}'(\cdot)$ that converts $\mathcal{X}'$ to $\mathcal{X}'_{prompt}$, where $\mathcal{X}_{prompt}'$ is an argument-enhanced input example by APM strategy and the prompt construction with the deliberate initializations, i.e., $\mathcal{X}'_{prompt} = \mathcal{T}'(\mathcal{X}')$.
Our final input structure for prompt-based fine-tuning is as follows:
\begin{equation}
    \scalebox{0.88}{$
    \begin{aligned}
    \mathcal{T'}(\mathcal{X}')=\text{``}&\texttt{[CLS]}D'\texttt{[SEP]}\texttt{[subj]}\tilde{a}_1\texttt{[subj]} \\
    &\texttt{[MASK]}\texttt{[obj]}\tilde{a}_2\texttt{[obj]}\texttt{[SEP]}\text{"}.
    \end{aligned}
    $}
\end{equation}
% where $x'$ is an argument-enhancing input example by AAE and prompt initialization, i.e., $x' =\{D',\tilde{a}_s, \tilde{a}_o\}$.
% For instance, relation `per:date\_of\_birth' is initialized by aggregating its metadata, \{`person', `date', `of', `birth'\}. 

% semantic answer tokens and map the mask token to the label by using label mapping function, i.e., verbalizer $\mathcal{V}$. $\mathcal{V}$ projects the mask token to representative relation token set. 


% For this, we define the semantic token set for relation $\mathcal{V}_{rel}$ which includes each semantic relation class, i.e.,
% \begin{equation} \label{equ:v_r}
%     \mathcal{V}_{rel} = \{ \text{`[per:date\_of\_birth]', `[gpe:residents\_of\_place]'}, \dots \}.
% \end{equation}

\input{tables/1. main experiments}
% For example, we use a special token \textit{[per:date\_of\_birth]} for the relation `per:date\_of\_birth'. 
% Init을 얘기하면서 potential words로 치환된 뒤, 각 embedding의 mean vector로 초기화한다를 아래에서 씀
% Moreover, the implicit semantics about the relation type are extracted from relation labels, that is, a relation label 이 일련의 semantic word set 으로 치환된다 such as `per:date\_of\_birth' to \{`date', `of', `birth'\}. 
% $\mathcal{C}^{rel}$ is a set of the semantic word sets for each relation label, where $\mathcal{C}^{rel}=$ \{\{`date', `of', `birth'\}, \{`place`, `of', `birth'\}, \dots\}
% We initialize the virtual token \textit{[per:date\_of\_birth]} by aggregating the embeddings of the semantic words. The specific equation is as follows:

% \begin{equation}
%     e'_{[rel]}(\mathcal{V}_{rel}(y)) = E[e(\mathcal{C}^{rel}(y))]
% \end{equation}

% where $e'_{[rel]}$ is a set of embedding of semantic tokens for relation, and $E[\cdot]$ is an operation for expected value.

\subsection{Relational Clue Detection task}\label{subsection:rcd}
To lift up the understanding capability on relational clues with prompt-based fine-tuning approach, we introduce a relational clue detection (RCD) task. We define a set of \textit{label words} $\mathcal{V}_{rcd}$ that are added into model's vocabulary as $\mathcal{V}_{rcd}=$\{\texttt{[subject]}, \texttt{[object]}, \texttt{[trigger]}, \texttt{[outside]}\}. 
% and a label sequence of relational clue types $\mathcal{Y}_{rcd}$, where 
Afterwards, we construct a label sequence for RCD, $\mathcal{C}_{rcd}$ by assigning each token in the $\mathcal{X}'_{prompt}$ to corresponding clue type word from $\mathcal{V}_{rcd}$.
% assign each token in $x'_{prompt}$ to corresponding clue type in $\mathcal{V}_{rcd}$.
% Each token in $\mathcal{Y}_{rcd}$ is assigned each token to corresponding clue type in $\mathcal{V}_{rcd}$ for RCD, where $\mathcal{V}_{rcd}=\{\texttt{[subject]}, \texttt{[object]}, \texttt{[trigger]}, \texttt{[outside]}\}$ and $\mathcal{M}_{rcd}:\mathcal{Y}_{rcd}\to\mathcal{V}_{rcd}$.
%  For MLM, we define $\mathcal{V}_{mlm}=\{\texttt{[per:data\_of\_birth]}, \cdots \}$ and $\mathcal{M}_{mlm}:y\to\mathcal{V}_{mlm}$.
% In detail, we define $\mathcal{V}_{rcd}=\{\texttt{subject}, \texttt{object}, \texttt{trigger}, \texttt{outside}\}$ and $\mathcal{M}_{rcd}:y\to\mathcal{V}_{rcd}$.
% Next, we define a mapping function $\mathcal{M}_{rcd}:\mathcal{C}_{rcd}\to\mathcal{V}_{rcd}$.
% In detail, all of the tokens are assigned with the label in $\mathcal{V}_{rcd}$ = \{``subject", ``object", ``trigger", ``outside"\}, which are a set of class words from model's vocabulary.
For instance, $\mathcal{C}_{rcd}$ is constructed like \{\texttt{[subject]}, \texttt{[trigger]}, \texttt{[object]}\} when the token sequence is given as $\{\textit{``Pheebs"}, \textit{``lives in"}, \textit{``LA"}\}$, where \textit{``Pheebs"} is a subject and \textit{``LA"} is an object argument, and \textit{``lives in"} is a trigger, respectively. 

% RCD는 추가 레이어 없이 [MASK]를 예측할때 사용하는 MLM head를 사용한다. In detail, RCD는 이 MLM head를 non-[MASK] token 에 해당하는 임베딩을 이용하여 sequence tagging을 진행하는 것이 목표다

RCD task exploits the MLM head that is used to predict the \texttt{[MASK]} token. By adopting the embeddings of the non-\texttt{[MASK]} indices, it sequentially tags each of the token with $\mathcal{V}_{rcd}$. 
In other words, the RCD task lets the model identify which non-\texttt{[MASK]} tokens corresponds to certain relational clue type. RCD supports the model to collect scattered information among the entire dialogue by indicating where to focus in the dialogue for predicting a relation. In this respect, the model pays far more attention to the semantic clues of the relation. Moreover, our model maintains its lightweight complexity by conducting RCD task without an additional classifier.
The loss for RCD task over each token is aggregated as follows:
% \begin{equation} \label{equ:rcd_loss}
%     \begin{aligned}
%         \mathcal{L}_{RCD} & = -\frac{1}{|\mathcal{X}'|}\sum_{x' \in \mathcal{X}',~c \in \mathcal{C}_{rcd}} \log \prod^N_{i=1}P(x_i=c|x'_{prompt}=\mathcal{T}(x'))  \\
%     \end{aligned}
% \end{equation}
\begin{equation} \label{equ:rcd_loss}
    \scalebox{0.9}{$\begin{aligned}
        \mathcal{L}_{RCD} & = -\sum_{x \in \mathcal{X}}\log P(\mathcal{C}_{rcd}(x)|\mathcal{X}'_{prompt})  \\
    \end{aligned}$}.
\end{equation}



\subsection{Model Training} \label{subsec:model_training}
% Multi-stage GRASP
Before the final relation prediction step, 
% the input is reconstructed based on the predicted results by the RCD task.
we mark the position of trigger using \texttt{[p]} token, i.e., APM marker, based on the result of the RCD task.
In detail, given example, $\mathcal{X}'_{prompt}$, the model predicts the clue type words for all of the non-mask tokens. Afterward, \texttt{[p]} is appended in front of the words predicted as a trigger to train the model to distinguish essential clues which help decide the relation.

\paragraph{Multi-task Learning}
$\mathcal{V}_{rel}$ refers to a set of \textit{label words} in the model's vocabulary for relation prediction in MLM manner as in Figure \ref{fig:model_overview}.
Then, $\mathcal{M}_{rel}:\mathcal{Y}\to\mathcal{V}_{rel}$ is an mapping function which converts a class set $\mathcal{Y}$ to a set of \textit{label words} $\mathcal{V}_{rel}$. 
For each input $\mathcal{X}'_{prompt}$, the purpose of MLM is to fill the \texttt{[MASK]} with the relation \textit{label words} in the model's vocabulary.
As the model predicts the correct \textit{label word} at the position of \texttt{[MASK]}, we can formulate $p(y|x)=P(\texttt{[MASK]}=\mathcal{M}_{rel}(y)|\mathcal{X'}_{prompt})$.
The training objective of the relation prediction is to minimize
% $\mathcal{L}_{REL}$ 에 대한 설명
\begin{equation} \label{MLM_loss}
    \scalebox{0.87}{$
    \mathcal{L}_{REL} & = -\log P(\texttt{[MASK]}=\mathcal{M}_{rel}(y)|\mathcal{X}'_{prompt}).
    $}
\end{equation}

% mtl
To improve the model's ability to capture the relational clues through the interaction between the MLM task for relation prediction and our RCD task,
we employ a multi-task learning to train $\mathbf{GRASP}$ model, and the joint loss for Equation.~(\ref{equ:rcd_loss}) and the Equation.~(\ref{MLM_loss}) is used. 
Therefore, the final learning objective is to minimize the joint loss, where $\lambda_{1}$ and $\lambda_{2}$ are hyperparameters.
\begin{equation} \label{final_loss}
    \scalebox{0.9}{$\mathcal{L}_{GRASP} = \lambda_{1} \cdot \mathcal{L}_{RCD} + \lambda_{2} \cdot \mathcal{L}_{REL}$}
\end{equation}


==> sections/3_experiments.tex <==
\section{Experiments\label{sec:experiments}}
\subsection{Experimental Setup}
% We adopt RoBERTa-base and RoBERTa-large to prompt-tune our approach, and denote as $\mathbf{GRASP}_{base}$ and $\mathbf{GRASP}_{large}$, respectively.
We adopt RoBERTa-base and RoBERTa-large as our base PLMs and denote them as $\mathbf{GRASP}_{base}$ and $\mathbf{GRASP}_{large}$, respectively.
For evaluation metric, We use both F1 and F1$_c$ \citep{yu-etal-2020-dialogue} scores. F1$_c$ is an evaluation metric for supplementing F1 score in a conversational setting, which is computed by employing a part of dialogue necessary for predicting the relation between given arguments as input instead of the entire dialogue. The detailed settings for our $\mathbf{GRASP}$ can be found in Appendix \ref{appendix:experiment_settings}.
% full-shot setting 에 대한 설명
In a full-shot setting, we compare $\mathbf{GRASP}$ with both fine-tuning based approaches and prompt-based fine-tuning approaches.
As fine-tuning baseline models, 
TUCORE-GCN~\citep{lee-choi-2021-graph} is the typical fine-tuning based model using turn-level features with graph convolution network~\cite{kipf2016semi}, CoIn~\citep{ijcai2021-535} employs utterance-aware and speaker-aware representations, 
and Dual~\cite{bai-etal-2021-semantic} models relational semantics using abstract meaning representation~\cite{banarescu-etal-2013-abstract}.
Moreover, PTR~\citep{han2021ptr} and KnowPrompt~\citep{chen2021knowprompt} are typical prompt-based fine-tuning baseline models.
In a few-shot setting, we conduct 8-, 16-, and 32-shot experiments following LM-BFF~\citep{gao2020making} based on three different randomly sampled data. 

\input{tables/few_shot}
\subsection{Experimental Results}
\paragraph{Full-shot setting}
As shown in Table \ref{tab:main_experiments}, the baselines on the fine-tuning based approach such as TUCORE-GCN or CoIn show better performance than those of the prompt-based fine-tuning approach. In particular, CoIn overwhelms all of the other baselines, including PTR and KnowPrompt on V1, and also TUCORE-GCN performs the best score on V2. This result illustrates that fine-tuning the models with complicated structures in the full-shot setting is substantial compared to the existing prompt-based fine-tuning approaches. 

However, even though $\mathbf{GRASP}_{large}$ is the prompt-based fine-tuning model, it surpasses over all the baseline models, even including the current SoTA model, i.e., CoIn and TUCORE-GCN.
% Table \ref{tab:main_experiments} demonstrates the performance of $\mathbf{GRASP}$ on the DialogRE dataset. From the result, it is found that our $\mathbf{GRASP}_{large}$ model performs better than any other baseline models including the current SoTA model, i.e. TUCORE-GCN.
In addition, $\mathbf{GRASP}_{large}$ shows its strength in conversational setting as well by exceeding all of the baselines in F1$_c$, thereby indicating that our method effectively overcome the low information density of dialogue.
These results imply guiding the model to pay attention to relational clues with a prompt-based fine-tuning approach is more effective than adding extra features and layers.
We assume that the slight lacking performance of $\mathbf{GRASP}_{base}$ can be derived from the gap in model size; for example, TUCORE-GCN has 401M weight parameters, and $\mathbf{GRASP}_{base}$ has 125M weight parameters. In fact, $\mathbf{GRASP}_{base}$ demonstrates 6.0\%p and 0.6\%p improvements compared to the other prompt-based fine-tuning baselines, i.e., PTR and KnowPrompt, respectively. 

\input{tables/grasp_ablation}
\input{tables/prompt_marker}
\input{tables/rcd_ablation}
\paragraph{Few-shot setting}
From Table \ref{table:few_shot}, $\mathbf{GRASP}$ is still exhibits robust performance in few-shot settings. $\mathbf{GRASP}_{base}$ outperforms the other baselines of both fine-tuning and prompt-based fine-tuning methods regardless of the number of shots.
In particular, it demonstrates more than 20\%p higher performance in 8-shot setting compared to TUCORE-GCN, suggesting that our method is more powerful than the fine-tuning method in the low-resource setting.
$\mathbf{GRASP}_{base}$ also shows improved performance compared to KnowPrompt in all shot settings, indicating the effectiveness of our considerations on the properties of dialogue with prompt-based fine-tuning.

Except for the 8-shot setting, $\mathbf{GRASP}_{large}$ shows outstanding performances; in particular, the achieves up to 15.3\%p of absolute improvement in the 16-shot setting. The reason for the limited performance of $\mathbf{GRASP}_{large}$ in the 8-shot setting can be attributed to the insufficient number of examples. 


We also observe that the fine-tuning based models such as TUCORE-GCN perform at least 5.7\%p worse than the prompt-based fine-tuning models such as PTR in 8-shot setting, which indicates that the fine-tuning based models may have difficulty of capturing relational semantics enough when the data are extremely scarce. In particular, TUCORE-GCN even shows 5.2\%p lower performance than the fine-tuned RoBERTa, thereby indicating that its high complexity requires a larger amount of data than the other models.

\paragraph{Ablation Study}
We conduct an ablation study to show the effectiveness of our proposed modules. In Table \ref{table:grasp_ablation}, each of our suggested modules improves the overall performances in both F1 and F1$_c$ settings. We first observe that without the APM strategy, the performance of $\mathbf{GRASP}_{base}$ drops by 0.8\%p F1 score and 0.4\%p F1$_c$ score on the development set and sharply drops by 2.1\%p F1 score and 1.0\%p F1$_c$ score on the test set. This result indicates that an argument-awareness can be obtained through both the speaker and non-speaker argument information.
When the RCD task is removed, the performance of $\mathbf{GRASP}_{base}$ decreases by 1.1\%p F1 score and 0.5\%p F1$_c$ score on the development set and decreases by 1.3\%p F1 score and 0.7\%p F1$_c$ score on the test set. This result demonstrates that the RCD task alleviates the low information density of dialogue by guiding the model to focus on relational clues.

Additionally, the performance without the manual initialization of prompt construction of $\mathbf{GRASP}_{base}$ is reduced by a 2.2\%p F1 score and 1.4\%p F1$_c$ score on the development set and is reduced by 3.1\%p F1 score and 1.9\%p F1$_c$ score on the test set. This result suggests that the prompt construction is a basic step to training the model in the prompt-based fine-tuning manner. The deliberate initialization of the prompts is critical to model tasks in an appropriate direction.

==> sections/4_analysis.tex <==
\input{tables/rcd_qualitative_analysis}
\section{Analysis}
\subsection{Analysis on marker type for APM}

In order to analyze argument-awareness regarding the types of marker, we conduct the experiments on diverse prompt markers as depicted in Table \ref{table:prompt_marker_analysis}. The result illustrates that the taking argument types into account leads to the performance improvement of the model. While the punctuation marker ``;'' shows the comparable performance among the punctuation markers, ``!'' and ``@'' achieves limited score. We may presume that the higher frequency of the ``;'' that acts as the delimiter. In other words, we may infer the meta-information on usage of punctuation drives the result. 
% Type marker가 Entity marker보다 좋은 성능을 보였는데, 이는 argument type을 고려하는 것이 약간의 성능 개선을 가져올 수 있음을 시사한다. Punctuation markers 중에서는 punctuation marker (;) marker가 가장 좋은 성능을 보였다. 이유는 ``;"가 다른 punctuations such as ``!" and ``@"보다 일반적으로 문장을 구분할 때 더 자주 사용되기 때문이라고 생각된다. 다시 말해서, punctuation의 general meta-information이 성능에 크게 작용했다고 보여진다.
% From the results, Type marker shows improvements compared with Entity marker, 

% The embedding of \texttt{[p]} in the APM method is initialized with the space token from the model's vocabulary.
We also observe that the APM marker (front) performs the best with a 75.5\% F1 score among all other marker types. In addition, we conduct experiment based on the position of the prompt marker \texttt{[p]} by comparing two versions of APM marker type, i.e., APM marker (front) and APM marker (surrounding).
The APM marker (surrounding) shows 2.7\%p lower performance compared to the APM marker (front). Following these results, we empirically adopt the embedding initialization of our \texttt{[p]} prompt marker using the space token.

\subsection{Analysis on the applicability of $\mathbf{GRASP}$}
To demonstrate the robustness of our APM strategy and RCD task, we additionally experiment $\mathbf{GRASP}$ on MELD~\cite{poria-etal-2019-meld} and EmoryNLP~\cite{zahiri2018emotion} datasets which are designed for emotion recognition in conversations (ERC). 
For baselines, we employ the fine-tuned RoBERTa~\cite{liu2019roberta}, COSMIC~\cite{ghosal-etal-2020-cosmic}, and TUCORE-GCN~\cite{lee-choi-2021-graph}. 
% TUCORE-GCN is the current SoTA model in DialogRE task.
The detailed information of the datasets and baseline used in this analysis is in the Appendix \ref{appendix:erc}.

From Table \ref{table:rcd_ablation}, we identify that $\mathbf{GRASP}$ is well applicable to other dialogue-based tasks by alleviating the low information density of given dialogue. In particular, $\mathbf{GRASP}$ shows the performances surpassing those of TUCORE-GCN which is the current SoTA model in DialogRE and those of the baseline specialized in ERC task such as COSMIC in both MELD and EmoryNLP.

\subsection{Qualitative Analysis on $\mathbf{GRASP}$}
\label{subsec:qualitative}

Since we trained $\mathbf{GRASP}$ attending on relational clues through the APM strategy and the RCD task, we further conducted analysis to investigate that the relational clues such as triggers contribute to predicting a relation between the arguments in a prompt-based manner, as shown in Table \ref{table:rcd_qualitative_analysis}. Specifically, we compared $\mathbf{GRASP}_{large}$ with a fine-tuned RoBERTa-large model to validate our method.

We observed that the fine-tuned RoBERTa model struggles to capture the symmetrical relations including the trigger. The fine-tuned RoBERTa model failed to capture relational clues, such as ``moving in together", misleading the model into predicting an inappropriate relation ``per:roommate" for both symmetrical relations between S2 and Chandler. ``moving in together" is a critical cue to distinguish the relations between ``per:roommate" and ``per:girl/boyfriend" because this phrase implies a romantic relationship in a dictionary definition. 
In contrast, $\mathbf{GRASP}$, which was trained using the RCD task and the APM strategy in a prompt-based manner, predicted the correct relations, capturing the correct relational clues including the trigger ``moving in together" for both symmetrical argument pairs. This result proves the effectiveness of $\mathbf{GRASP}$ designed to guide the model on the relational clues, alleviating the difficulties of low information density in dialogues.
Additional examples demonstrating similar phenomena for the symmetrical relations are provided in the Appendix \ref{appendix:qualitative}.


==> sections/5_conclusions.tex <==

\section{Conclusion}
% [요약 - 결과 - 향후 전망]
% 요약
In this paper, we proposed $\mathbf{GRASP}$, which is the way of guiding PLMs to relational semantics using prompt-based fine-tuning for DialogRE task. We concentrated on alleviating the critical challenge of dialogue, i.e., low information density, by effectively capturing the relational clues.
In $\mathbf{GRASP}$, we first constructed prompts with deliberate initialization and suggest 1) an argument-aware prompt marker (APM) strategy with the consideration on both speaker and non-speaker arguments and 2) the relational clue detection (RCD) task which guides the model to discriminate which token belongs to the relational clues. 
For experiments, 
Experimental results on the DialogRE dataset demonstrated that $\mathbf{GRASP}$ achieved the SoTA performance at F1 and F1$_c$ scores, even though our method only leveraged a PLM without adding any extra layer.
In addition, from experimental results on the ERC datasets, $\mathbf{GRASP}$ proved its applicability to other dialogue-based tasks.
% 향후 전망
We hope that this study will suggest the possibility that a simple and effective method such as $\mathbf{GRASP}$ reasonably deals with complex tasks such as DialogRE and ERC. 
% in which multiple speakers appear and considerations in a wide range for finding answers are required.


==> tables/gggg_ablation.tex <==
% \begin{table*}[t]
% \centering
% \begin{tabular}{l|cl|cc|cc@{}}
% \toprule
%       & \multicolumn{2}{c|}{\textbf{No marker}} & \multicolumn{2}{c|}{\textbf{Start token}} & \multicolumn{2}{c}{\textbf{All of tokens}} \\
%       & \multicolumn{2}{c|}{-}                  & front                & back               & front                & back                \\ \midrule
% F1    & \multicolumn{2}{c|}{73.8}               &          \textbf{83.3}            &        82.7            &       81.7               &            \textbf{83.3}         \\
% F1$_c$ & \multicolumn{2}{c|}{66.5}                   &           \textbf{73.8}           &        73.0            &           72.2           &            72.7         \\ \bottomrule
% \end{tabular}
% \label{table:gggg_ablation} 
% \caption{Performances (F1 and F1$_c$) comparison of methods
% with considering the source of entity marker prompt.}
% \end{table*}

\begin{table*}[t]
\centering
\scalebox{1.0}{
\begin{tabular}{l|cl|cc|cc@{}}
\toprule
      & \multicolumn{2}{c|}{\textbf{No marker}} & \multicolumn{2}{c|}{\textbf{Start token}} & \multicolumn{2}{c}{\textbf{All of tokens}} \\
      & \multicolumn{2}{c|}{-}                  & front                & back               & front                & back                \\ \midrule
F1    & \multicolumn{2}{c|}{73.8}               &          \textbf{83.3} (+9.5)            &        82.7 (+8.9)            &       81.7 (+7.9)               &            \textbf{83.3} (+9.5)         \\
F1$_c$ & \multicolumn{2}{c|}{66.5}                   &           \textbf{73.8} (+7.3)           &        73.0 (+6.5)            &           72.2 (+5.7)          &            72.7 (+6.2)        \\ \bottomrule
\end{tabular}
}
\caption{Performances (F1 and F1$_c$) comparison of methods
with considering the source of entity marker prompt. Note that the number in parentheses is the performance increase compared to ``No marker".\label{table:gggg_ablation} }
\end{table*}

==> tables/prompt_where_to_locate.tex <==
\begin{table}[ht]
\centering
\scalebox{0.9}{
\begin{tabular}{l|l|l}
\toprule
\textbf{Marker Position} & \textbf{Input Example} & \textbf{F1} \\ \midrule
Front                    & \texttt{[p]} Frank & 84.7            \\
Surrounding              & \texttt{[p]} Frank \texttt{[p]} & 74.4            \\ \bottomrule
\end{tabular}
}
\caption{The performance of APM strategy according to the position of the prompt marker\label{table:prompt_where_to_locate}}
\end{table}



